UniGuard: Towards Universal Safety Guardrails for Jailbreak Attacks on Multimodal Large Language Models

Multimodal large language models (MLLMs) have revolutionized vision-language understanding but remain vulnerable to multimodal jailbreak attacks, where adversarial inputs are meticulously crafted to elicit harmful or inappropriate responses. We propose UniGuard, a novel multimodal safety guardrail that jointly considers the unimodal and cross-modal harmful signals. UniGuard trains a multimodal guardrail to minimize the likelihood of generating harmful responses in a toxic corpus. The guardrail can be seamlessly applied to any input prompt during inference with minimal computational costs. Extensive experiments demonstrate the generalizability of UniGuard across multiple modalities, attack strategies, and multiple state-of-the-art MLLMs, including LLaVA, Gemini Pro, GPT-4o, MiniGPT-4, and InstructBLIP. Notably, this robust defense mechanism maintains the models' overall vision-language understanding capabilities.

==> src/fig/fig-mmvet_varying_eps.tex <==
\begin{figure}[!h]
    \centering
    \includegraphics[width=0.98\linewidth]{fig/fig_MM-Vet_varying_eps.pdf}
    \caption{}
    \label{fig:mmvet_varying_eps}
    \vspace{-3mm}
\end{figure}

==> tables/tab-ablation-study.tex <==

\begin{table*}[!ht]
    \centering
    \resizebox{1.0\linewidth}{!}{%
    \begin{tabular}{l cc cc cc cc cc}
    \toprule
     {\sc \textbf{Methods/Metrics}} & \multicolumn{6}{c}{\sc \textbf{Perspective API} (\%)} & \multicolumn{1}{c}{\sc \textbf{Fluency} } \\
    \cmidrule(lr){2-7} \cmidrule(lr){8-8} 
     & \begin{tabular}{@{}c@{}}\textbf{Attack} \\ \textbf{Success} \end{tabular} $\boldsymbol{\downarrow}$  & \begin{tabular}{@{}c@{}}Identity \\ Attack \end{tabular} $\boldsymbol{\downarrow}$ & Profanity $\boldsymbol{\downarrow}$ & \begin{tabular}{@{}c@{}}Sexually \\ Explicit \end{tabular}  $\boldsymbol{ \downarrow}$ & Threat $\boldsymbol{ \downarrow}$ & Toxicity $\boldsymbol{\downarrow}$ &  Perplexity $\boldsymbol{\downarrow}$\\
    \midrule
     No Defense & 81.61 & 25.41 & 67.22 & 39.38 & 40.64 & 77.93 & 21.84\\    
    \midrule 
    \textbf{Image Safety Guardrail Only} & \multicolumn{7}{c}{} \\ 
    \method (w/o text) ($\epsilon=\frac{32}{255}$) & 53.67 & 6.18 & 42.99 & 17.95 & 8.01 & 47.66 & 93.2\\
    \method (w/o text)  ($\epsilon=\frac{64}{255}$) & 38.78 & 3.00 & 30.11 & 9.09 & 3.17 & 31.94 & 5.04 \\
    \midrule 
    \textbf{Text Safety Guardrail Only} & \multicolumn{7}{c}{} \\ 
     \method (O w/o img) ($L=16$)  & 56.21 & 12.84 & 48.81 & 23.47 & 21.85 & 48.72 & 87.6 \\
     \method (O w/o img) ($L=32$)  & 60.24 & 13.23 & 46.93 & 25.78 & 22.83 & 51.73 & 25.1 \\
     \method (P w/o img) & 67.36 & 16.86 & 54.51 & 27.21 & 32.72 & 62.19 & 8.39 \\
    \midrule
    \textbf{Multimodal Safety Guardrails} & \multicolumn{7}{c}{} \\ 
    \method (O) & \textbf{25.17} & \underline{2.06} & \underline{22.34} & \underline{7.99} & \textbf{0.86} & \underline{\textbf{19.16}} & \underline{6.16}  \\
    \method (P) & \underline{25.69} & \textbf{1.58} &  \textbf{19.68} &  \textbf{7.01}  & \underline{1.50} & \underline{19.35} & \textbf{4.90} \\
    \bottomrule
    \end{tabular}%
    }
    \caption{Effectiveness of \method against \underline{unconstrained} visual attack~\citep{qi2023visual} and Real Toxicity Prompts (RTP)~\citep{gehman2020realtoxicityprompts} adversarial text on \llava 1.5. \method (w/o text) indicates only applying image guardrail, and \method (O w/o img) indicates only applying text guardrail. `$\downarrow$' means that lower values indicate better performances. The best and second best performances are highlighted in \textbf{bold} and \underline{underlined}, respectively. \method with multimodal safety guardrails shows the best robustness.}
    \label{tab:exp:ablation_study}
\end{table*} 
